Asymptotic rigidity of scaling ratios for critical circle mappings

In this paper we establish $C^2$ a-priori bounds for the scaling ratios of critical circle mappings in a form that gives also a compactness property for the renormalization operator.

==> abstrac1.tex <==
%auto-ignore
\baselineskip=10pt
\def\squeez{\parshape=2 27truemm 110truemm 27truemm 110truemm}
\squeez{\medtype
{\ni
\hsize=4 truein
{\bf Abstract.} In this paper we establish $C^2$ a-priori bounds for the
scaling ratios of critical circle mappings in a form that gives also
a compactness property for the renormalization operator.}

{\ni
\hsize=4 truein
{\bf Keywords.} Scaling ratios, Poincar\'e metric, renormalization.
}}



==> abstract.tex <==
%auto-ignore
\baselineskip=10pt
\def\squeez{\parshape=2 27truemm 110truemm 27truemm 110truemm}
\squeez{\medtype
{\ni
\hsize=4 truein
{\bf Abstract.} In this paper we establish $C^2$ a-priori bounds for the
scaling ratios of critical circle mappings in a form that gives also
a compactness property for the renormalization operator.
}}



==> fig1.tex <==
%auto-ignore
\input pictex
$$
\beginpicture
\setcoordinatesystem units <.7in,.35in>
\setplotarea x from -3.75 to 3.75 , y from -1.5 to 4.0
\setplotsymbol({\fiverm .})
\plot -3.5 1.1 3.5 1.1 /
\plot -1.3 -1.15 1.3 3.35 /
\plot -1.3 3.35 1.3 -1.15 /
\put{$0$} at 0 .8 
\put{$a$} at -1.8 .8
\put{$b$} at 1.8 .8
\put{$\eta(0)$} at -.6 .8
\put{$\xi(0)$} at 1.2 .8
\put{$Re\,z$} at 3.4 .8
\put{${\cal O}_\xi$} at -1.7 3.1
\put{${\cal O}_\eta$} at 1.7 3.1
\put{${\cal O}_\nu$} at 0 -1.1
\put{${\cal D}$} at 2.4 3.75
\put{\it Figure 1} at 0 -3.5
\put{$\xi$} at -.9 3.45
\put{$\eta$} at .9 3.45
\put{$\nu$} at .55 -1.2
\arrow  <6pt> [.2, .7]  from  -1.3 2.75 to -.7 3.31
\arrow  <6pt> [.2, .7]  from  1.3 2.75 to .7 3.31
\arrow  <6pt> [.2, .7]  from  .6 .7 to .4 -1.2
\circulararc 82 degrees from -1.3 3.35 center at 0 1.1
\circulararc 82 degrees from 1.3 -1.15 center at 0 1.1
\circulararc 360 degrees from .95 1.1 center at 0 1.1
\ellipticalarc axes ratio 3:2 360 degrees from 2.8 1.1 center at 0 1.1
\setplotsymbol({\tenrm .})
\arrow  <6pt> [.2, .7]  from  1.2 1.1 to 3.5 1.1
\plot -3.5 1.1 -.6 1.1 /
\put{$\scriptstyle\circ$} at -.6 1.1
\put{$\scriptstyle\circ$} at 1.2 1.1
\put{$\scriptstyle\circ$} at 0 1.1
\endpicture
$$


==> fig2.tex <==
%auto-ignore
\input pictex
$$
\beginpicture
\setcoordinatesystem units <.78in,.8in>
\setplotarea x from -3.0 to 3.0 , y from -1 to 4
\setplotsymbol({\fiverm .})
\arrow  <6pt> [.2, .7]    from  -2.95 0 to 2.95 0
\put{\it Figure 2} at 0 -.7
\put{$0$} at 0 -.15
\put{$1$} at .9 -.15
\put{$-1$} at -.98 -.15
\put{$p_n$} at 1.8 -.15
\put{$Re\,z$} at 2.9 -.15
\put{$\alpha_n$} at -.69 -.15
\put{$\beta_n$} at .7 -.15
\put{$A_{n,R}$} at -.3 .26
\put{$B_{n,R}$} at .3 .26
\put{$V_0$} at -.7 2.9
\put{$V_1$} at .2 2.9
\put{$V_{p_n+1}$} at 1.9 2.9
\put{$y=\delta(|x|,2R)$} at -1.4 1.2
\put{${\cal D}_R^{+}$} at -1.7 2.4
\circulararc 180 degrees from 2.8 0 center at 0 0
\setplotsymbol({\sevenrm .})
\setquadratic
%Increasing 
\plot -2.7 0 -2.5 .8  -2.3 3.0 /
%\plot -1.8 0 -1.6 .8  -1.4 3.0 /
\plot -.9 0 -.7 .8  -.5 3.0 /
\plot 0 0 .2 .8  .4 3.0 /
%\plot 0.9 0 1.1 .8  1.3 3.0 /
\plot 1.8 0 2.0 .8  2.2 3.0 /
%Decreasing
\plot -2.2 3.0 -2.0 .8 -1.8 0 /
%\plot -1.3 3.0 -1.1 .8 -.9 0 /
\plot -.4 3.0 -.2 .8 0 0 /
\plot .5 3.0 .7 .8 0.9 0 /
%\plot 1.4 3.0 1.6 .8 1.8 0 /
\plot 2.3 3.0 2.5 .8 2.7 0 /
%Logarithmic cut-off
\plot -2.8 1.2 -1.9 1.1 -1.0 .9 /
\plot 1.0 .9 1.9 1.1 2.8 1.2 /
\plot -1.0 .9 0 .9 1.0 .9 /
\setshadegrid span  <1 pt>
%\vshade .5 2.4 3 .8 1.9 2.5 1.1 1.2 2.1 /
%\hshade 0 1.8 2.3 .55 1.92 2.42 1.1 2.0 2.5 /
%\setplotsymbol({\tenrm .})
\plot -.7 0 -.575 .1 -.45 .5 /
\plot  -.45 .5 -.4 .54 -.35 .65 /
\plot  -.35 .65 -.325 .65 -.3 .65 /
\plot  -.3 .65 -.225 .48 -.15 .42 /
%\plot  -.15 .42 -.075 .155 0 0 /
%\plot  -.65 0 -.325 0 0 0 /
\plot .45 .5 .575 .1 .7 0 /
\plot  .35 .65 .4 .54 .45 .5 /
\plot  .3 .65 .325 .65 .35 .65 /
\plot  .15 .42 .225 .48 .3 .65 /
\setlinear
%\vshade .5 2.4 3 .8 2.4 3 /
%\vshade 1.09 1.2 1.7  1.36 1.7 1.7 /
\endpicture
$$


==> holomin.tex <==
%auto-ignore
CHAPTER II 
 
Holomorphic Commuting Pairs and Renormalization 
 
In this chapter we introduce a class of holomorphic dynamical systems 
together with a suitably defined renormalization operator acting on it. 
Such dynamical systems - which we baptize holomorphic commuting pairs 
- arise as natural extensions to the complex plane of certain real  
analytic commuting pairs (in the sense of Lanford), which in turn  
correspond to critical circle homeomorphisms with a singularity of cubic 
exponent-type. The operator acting on them restricts to the usual real 
renormalization operator of chapter I, as one might expect. 
 
After presenting a few basic properties of holomorphic commuting pairs, 
as well as some quasiconformal pre-requisites, we state and prove (\S 3) 
a pull-back type theorem that allows us, among other things, to  
transfer the real renormalization bounds developed in chapter I to this 
complex analytic context. 
 
Subsequently (\S 4), we define the Teichm\"uller space of a holomorphic 
commuting pair. Its elements correspond to quasiconformal deformations 
of the given object which are later shown (\S 5) to be entirely supported 
in the non-recurrent part of the associated dynamical system. This is  
accomplished by: first, showing that in some sense all renormalizations  
coming from mappings in the classical Arnold-Herman family (see M. Herman 
[H]) are holomorphic commuting pairs; second, proving the desired  
rigidity properties for that family; and third, using the results of  
\S 3 to spread this information over to all holomorphic commuting pairs. 
Notice that the question of existence of such objects is settled {\it en  
passant}. 
 
We close these remarks with a few words on notation that pervades this 
chapter. If $I \subseteq \R$ is an interval, we write ${\bf C}(I)$ to  
denote ${\bf C} - (\R - {\rm int}(I))$. An expression such as  
$f : A \rt\!\!\!\!\rt B$ means that $f$ is onto $B$, and is used whenever 
we want to emphasize surjectivity somehow. All covering mappings  
appearing in the text, branched or unbranched, will be regular coverings. 
Finally, if $A \subseteq {\bf C}$ then $A^+$ denotes the set of all  
$z \in A$ such that ${\rm Im}\,z > 0$, and $A^-$ is similarly defined.










==> psbox.tex <==
%% Every macro likes a little privacy...
\catcode`\@=11


                  %% -------------------------- %%


%%
%% Trying to tame the variety of \special commands for Postscript: the
%% universal internal command \PSspeci@l##1##2 takes ##1 to be the
%% filename and ##2 to be the integer scale factor*1000 (as for usual
%% TeX \scale commands)
%

\def\psfortextures{%     For TeXtures on the Macintosh
\def\PSspeci@l##1##2{%
\special{illustration ##1\space scaled ##2}}}

                          %% ----------- %%

\def\psfordvips{%      For DVIPS converter on VAX, UNIX and PC's
\def\PSspeci@l##1##2{%
\d@my=0.1bp \d@mx=\drawingwd \divide\d@mx by\d@my%
\special{PSfile=##1\space llx=\psllx\space lly=\pslly\space%
urx=\psurx\space ury=\psury\space rwi=\number\d@mx}}}

                          %% ----------- %%

%%
%% Correspond parfaitement a la doc OzTeX.
%% 
\def\psforoztex{%        For the OzTeX shareware on the Macintosh
\def\PSspeci@l##1##2{%
\special{##1 \space
      ##2 1000 div dup scale
      \putsp@ce{\number-\psllx} \putsp@ce{\number-\pslly} translate}}}
\def\putsp@ce#1{#1 }

                          %% ----------- %%

\def\psonlyboxes{%     Draft-like behaviour if none of the others works
\def\PSspeci@l##1##2{%
\at{0cm}{0cm}{\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at{0cm}{0cm}{\hbox{(##1)}}\hss}
  }}}}}


                  %% -------------------------- %%


%%
%% \ReadPSize{PSfilename} reads the dimensions of a PostScript drawing
%% and stores it in \drawinght(wd)
%%
\newdimen\drawinght\newdimen\drawingwd
\newdimen\psxoffset\newdimen\psyoffset
\newbox\drawingBox

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%%
\pspoints=1bp          % Adobe points are `big'
\epsfxsize=0pt         % Default value, means `use natural size'
\epsfysize=0pt         % ditto


\def\ReadPSize#1{
\edef\PSfilename{#1}
\global\def\epsfllx{72}
\global\def\epsflly{72}
\global\def\epsfurx{540}
\global\def\epsfury{720}
%%
%%   The first thing we need to do is to open the
%%   PostScript file, if possible.
%%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%%
%%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%%   start with %. We're looking for the bounding box comment.
%%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%%
%%   We check to see if the first character is a % sign;
%%   if not, we stop reading (unless the line was entirely blank);
%%   if so, we look further and stop only if the line begins with
%%   `%%BoundingBox:'.
%%
          \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi
\def\psllx{\epsfllx}\def\pslly{\epsflly}%
\def\psurx{\epsfurx}\def\psury{\epsfury}%
%% Units related by crazy factors as bp/pt=72.27/72 should be BANNED!
\drawinght=\epsfury bp%
\advance\drawinght by-\epsflly bp%
\drawingwd=\epsfurx bp%
\advance\drawingwd by-\epsfllx bp%
}

%%
%%   We still need to define the tricky \epsfaux macro. This requires
%%   a couple of magic constants for comparison purposes.
%%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%%
%%   So we're ready to check for `%BoundingBox:' and to grab the
%%   values if they are found.
%%
%% \long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
%%    \def\testit{#2}\ifx\testit\epsfbblit
%%       \epsfgrab #3 . . . \\%
%%       \epsffileokfalse
%%       \global\epsfbbfoundtrue
%%    \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 @ @ @ \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
   \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%

%%
%%   Here we grab the values and stuff them in the appropriate definitions.
%%
%% \def\epsfgrab #1 #2 #3 #4 #5\\{%
%%    \global\def\epsfllx{#1}\ifx\epsfllx\empty
%%       \epsfgrab #2 #3 #4 #5 .\\\else
%%    \global\def\epsflly{#2}%
%%    \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
   \global\def\epsfllx{#1}\ifx\epsfllx\empty
      \epsfgrab #2 #3 #4 #5 @\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%


                  %% -------------------------- %%


%%
%% \psboxto(xdim;ydim){psfilename}: you specify the dimensions and
%%    TeX uniformly scales to fit the largest one. If xdim=0pt, the
%%    scale is fully determined by ydim and vice versa.
%%    Notice: psboxes are a real vboxes; couldn't take hbox otherwise all
%%    indentation and all cr's would be interpreted as spaces (hugh!).
%%
\newcount\xscale \newcount\yscale \newdimen\pscm\pscm=1cm
\newdimen\d@mx \newdimen\d@my
\let\ps@nnotation=\relax
\def\psboxto(#1;#2)#3{\vbox{
   \catcode`\:=12
   \ReadPSize{#3}
   \divide\drawingwd by 1000
   \divide\drawinght by 1000
   \d@mx=#1
   \ifdim\d@mx=0pt\xscale=1000
         \else \xscale=\d@mx \divide \xscale by \drawingwd\fi
   \d@my=#2
   \ifdim\d@my=0pt\yscale=1000
         \else \yscale=\d@my \divide \yscale by \drawinght\fi
   \ifnum\yscale=1000
         \else\ifnum\xscale=1000\xscale=\yscale
                    \else\ifnum\yscale<\xscale\xscale=\yscale\fi
              \fi
   \fi
   \divide \psxoffset by 1000\multiply\psxoffset by \xscale
   \divide \psyoffset by 1000\multiply\psyoffset by \xscale
   \global\divide\pscm by 1000
   \global\multiply\pscm by\xscale
   \multiply\drawingwd by\xscale \multiply\drawinght by\xscale
   \ifdim\d@mx=0pt\d@mx=\drawingwd\fi
   \ifdim\d@my=0pt\d@my=\drawinght\fi
\message{[#3\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
 \hbox to\d@mx{\hss\vbox to\d@my{\vss
   \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
      \kern-\psyoffset
      \PSspeci@l{\PSfilename}{\the\xscale}
      \vss}\hss\ps@nnotation}
   \global\ht\drawingBox=\the\drawinght
   \global\wd\drawingBox=\the\drawingwd
   \baselineskip=0pt
   \copy\drawingBox
 \vss}\hss}
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%% \psboxscaled{scalefactor*1000}{PSfilename} allows to bypass the
%%   rounding errors of TeX integer divisions for situations where the
%%   TeX box should fit the original BoundingBox with a precision better
%%   than 1/1000.
%%
\def\psboxscaled#1#2{\vbox{
  \catcode`\:=12
  \ReadPSize{#2}
  \xscale=#1
  \divide\drawingwd by 1000\multiply\drawingwd by\xscale
  \divide\drawinght by 1000\multiply\drawinght by\xscale
  \divide \psxoffset by 1000\multiply\psxoffset by \xscale
  \divide \psyoffset by 1000\multiply\psyoffset by \xscale
  \global\divide\pscm by 1000
  \global\multiply\pscm by\xscale
\message{[#2\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
  \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
     \kern-\psyoffset
     \PSspeci@l{\PSfilename}{\the\xscale}
     \vss}\hss\ps@nnotation}
  \global\ht\drawingBox=\the\drawinght
  \global\wd\drawingBox=\the\drawingwd
  \baselineskip=0pt
  \copy\drawingBox
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%%  \psbox{PSfilename} makes a TeX box having the minimal size to
%%      enclose the picture
\def\psbox#1{\psboxscaled{1000}{#1}}


                  %% -------------------------- %%

%%
%%  Annotations & Captions etc...
%%
%% \centinsert{anybox} is just a centered \midinsert, but is included as
%% people barely use the original inserts from TeX.
%%
\def\centinsert#1{\midinsert\line{\hss#1\hss}\endinsert}
\def\psannotate#1#2{\def\ps@nnotation{#2\global\let\ps@nnotation=\relax}#1}
\def\pscaption#1#2{\vbox{
   \setbox\drawingBox=#1
   \copy\drawingBox
   \vskip\baselineskip
   \vbox{\hsize=\wd\drawingBox\setbox0=\hbox{#2}
     \ifdim\wd0>\hsize
       \noindent\unhbox0\tolerance=5000
    \else\centerline{\box0}
    \fi
}}}


                  %% -------------------------- %%


%%
%% \at{#1}{#2}{#3} puts #3 at #1-higher and #2-right of the current
%%    position without moving it (to be used in annotations).
%%
\def\at#1#2#3{\setbox0=\hbox{#3}\ht0=0pt\dp0=0pt
  \rlap{\kern#1\vbox to0pt{\kern-#2\box0\vss}}}


                  %% -------------------------- %%


%%
%% \gridfill(ht;wd) makes a 1cm*1cm grid of ht by wd whose lower-left
%%   corner is the current point
%%
\newdimen\gridht \newdimen\gridwd
\def\gridfill(#1;#2){
  \setbox0=\hbox to 1\pscm
  {\vrule height1\pscm width.4pt\leaders\hrule\hfill}
  \gridht=#1
  \divide\gridht by \ht0
  \multiply\gridht by \ht0
  \advance \gridht by \ht0
  \gridwd=#2
  \divide\gridwd by \wd0
  \multiply\gridwd by \wd0
  \advance \gridwd by \wd0
  \vbox to \gridht{\leaders\hbox to\gridwd{\leaders\box0\hfill}\vfill}}


                  %% -------------------------- %%


%%
%% Useful to measure where to put annotations
%%
\def\fillinggrid{\at{0cm}{0cm}{\vbox{\gridfill(\drawinght;\drawingwd)}}}


                  %% -------------------------- %%


%%
%% \frameit{\thick}{\skip}{\anybox}
%%    draws with thickness \thick a box around \anybox, leaving \skip of
%%    blank around it. eg \frameit{0.5pt}{1pt}{\hbox{hello}}
%% \boxit{\anybox} is a shortcut.
%%
\def\frameit#1#2#3{\hbox{\vrule width#1\vbox{
  \hrule height#1\vskip#2\hbox{\hskip#2\vbox{#3}\hskip#2}%
        \vskip#2\hrule height#1}\vrule width#1}}
\def\boxit#1{\frameit{0.4pt}{0pt}{#1}}


                  %% -------------------------- %%


\catcode`\@=12 % cs containing @ are unreachable

